Strain-induced quantum phase transitions in magic angle graphene

We investigate the effect of uniaxial heterostrain on the interacting phase diagram of magic-angle twisted bilayer graphene. Using both self-consistent Hartree-Fock and density-matrix renormalization group calculations, we find that small strain values ($\epsilon \sim 0.1 - 0.2 \%$) drive a zero-temperature phase transition between the symmetry-broken Kramers intervalley-coherent insulator and a nematic semi-metal. The critical strain lies within the range of experimentally observed strain values, and we therefore predict that strain is at least partly responsible for the sample-dependent experimental observations.

==> Figures/App_Fig_KIVC_Ly_scaling/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such a sff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 8
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.2     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
legend.handletextpad : 0.4    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
legend.columnspacing : 1.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.14 # the left side of the subplots of the figure
figure.subplot.right   : 0.9    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.17    # the bottom of the subplots of the figure
figure.subplot.top     : 0.99    # the top of the subplots of the figure
figure.subplot.wspace  : 0.32    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.2   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/App_Fig_KIVC_TIVC/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 8
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.2     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
legend.handletextpad : 0.4    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
legend.columnspacing : 1.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.05 # the left side of the subplots of the figure
figure.subplot.right   : 0.89    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.17    # the bottom of the subplots of the figure
figure.subplot.top     : 0.99    # the top of the subplots of the figure
figure.subplot.wspace  : 0.32    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.2   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/App_Fig_MPO_SV_spectra/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 8
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.1     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
legend.handletextpad : 0.4    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
legend.columnspacing : 1.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.16 # the left side of the subplots of the figure
figure.subplot.right   : 0.96    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.17    # the bottom of the subplots of the figure
figure.subplot.top     : 0.96    # the top of the subplots of the figure
figure.subplot.wspace  : 0.32    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.2   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/App_Fig_Phiy_scan/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 8
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.1     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
legend.handletextpad : 0.4    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
legend.columnspacing : 1.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.14 # the left side of the subplots of the figure
figure.subplot.right   : 0.97    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.17    # the bottom of the subplots of the figure
figure.subplot.top     : 0.99    # the top of the subplots of the figure
figure.subplot.wspace  : 0.32    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.2   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/Figure_nu_-2/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 8
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.1     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
legend.handletextpad : 0.4    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
legend.columnspacing : 1.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.105 # the left side of the subplots of the figure
figure.subplot.right   : 0.99    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.18    # the bottom of the subplots of the figure
figure.subplot.top     : 0.99    # the top of the subplots of the figure
figure.subplot.wspace  : 0.32    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.2   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/Figure_nu_-2/v0/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 9
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.2     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
#legend.handletextpad : 0.8    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
#legend.columnspacing : 2.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.15 # the left side of the subplots of the figure
figure.subplot.right   : 0.97    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.08    # the bottom of the subplots of the figure
figure.subplot.top     : 0.97    # the top of the subplots of the figure
figure.subplot.wspace  : 0.50    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.3   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/Figure_nu_-2/v1/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 9
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.2     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
#legend.handletextpad : 0.8    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
#legend.columnspacing : 2.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.11 # the left side of the subplots of the figure
figure.subplot.right   : 0.99    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.08    # the bottom of the subplots of the figure
figure.subplot.top     : 0.99    # the top of the subplots of the figure
figure.subplot.wspace  : 0.50    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.3   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.


==> Figures/Figure_nu_-2/v2/matplotlibrc <==
### MATPLOTLIBRC FORMAT

# This is a sample matplotlib configuration file - you can find a copy
# of it on your system in
# site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
# there, please note that it will be overwritten in your next install.
# If you want to keep a permanent local copy that will not be
# overwritten, place it in the following location:
# unix/linux:
#     $HOME/.config/matplotlib/matplotlibrc or
#     $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
# other platforms:
#     $HOME/.matplotlib/matplotlibrc
#
# See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
# more details on the paths which are checked for the configuration file.
#
# This file is best viewed in a editor which supports python mode
# syntax highlighting. Blank lines, or lines starting with a comment
# symbol, are ignored, as are trailing comments.  Other lines must
# have the format
#    key : val # optional comment
#
# Colors: for the color values below, you can either use - a
# matplotlib color string, such as r, k, or b - an rgb tuple, such as
# (1.0, 0.5, 0.0) - a hex string, such as ff00ff or #ff00ff - a scalar
# grayscale intensity such as 0.75 - a legal html color name, e.g., red,
# blue, darkslategray

#### CONFIGURATION BEGINS HERE

# The default backend; one of GTK GTKAgg GTKCairo GTK3Agg GTK3Cairo
# CocoaAgg MacOSX Qt4Agg Qt5Agg TkAgg WX WXAgg Agg Cairo GDK PS PDF SVG
# Template.
# You can also deploy your own backend outside of matplotlib by
# referring to the module name (which must be in the PYTHONPATH) as
# 'module://my_backend'.
#backend      : MacOSX

# If you are using the Qt4Agg backend, you can choose here
# to use the PyQt4 bindings or the newer PySide bindings to
# the underlying Qt4 toolkit.
#backend.qt4 : PyQt4        # PyQt4 | PySide

# Note that this can be overridden by the environment variable
# QT_API used by Enthought Tool Suite (ETS); valid values are
# "pyqt" and "pyside".  The "pyqt" setting has the side effect of
# forcing the use of Version 2 API for QString and QVariant.

# The port to use for the web server in the WebAgg backend.
# webagg.port : 8888

# If webagg.port is unavailable, a number of other random ports will
# be tried until one that is available is found.
# webagg.port_retries : 50

# When True, open the webbrowser to the plot that is shown
# webagg.open_in_browser : True

# When True, the figures rendered in the nbagg backend are created with
# a transparent background.
# nbagg.transparent : True

# if you are running pyplot inside a GUI and your backend choice
# conflicts, we will automatically try to find a compatible one for
# you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   # None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        # a pytz timezone string, e.g., US/Central or Europe/Paris

# Where your matplotlib data lives if you installed to a non-default
# location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


### LINES
# See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
# information on line properties.
lines.linewidth   : 1.25     # line width in points
#lines.linestyle   : -       # solid line
#lines.color       : blue    # has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    # the default marker
#lines.markeredgewidth  : 0.5     # the line width around the marker symbol
lines.markersize  : 4            # markersize, in points
#lines.dash_joinstyle : miter        # miter|round|bevel
#lines.dash_capstyle : butt          # butt|round|projecting
#lines.solid_joinstyle : miter       # miter|round|bevel
#lines.solid_capstyle : projecting   # butt|round|projecting
#lines.antialiased : True         # render lines in antialiased (no jaggies)

#markers.fillstyle: full # full|left|right|bottom|top|none

### PATCHES
# Patches are graphical objects that fill 2D space, like polygons or
# circles.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
# information on patch properties
#patch.linewidth        : 1.0     # edge width in points
#patch.facecolor        : blue
#patch.edgecolor        : black
#patch.antialiased      : True    # render patches in antialiased (no jaggies)

### FONT
#
# font properties used by text.Text.  See
# http://matplotlib.org/api/font_manager_api.html for more
# information on font properties.  The 6 font properties used for font
# matching are given below with their default values.
#
# The font.family property has five values: 'serif' (e.g., Times),
# 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
# 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
# these font families has a default list of font names in decreasing
# order of priority associated with them.  When text.usetex is False,
# font.family may also be one or more concrete font names.
#
# The font.style property has three values: normal (or roman), italic
# or oblique.  The oblique style will be used for italic, if it is not
# present.
#
# The font.variant property has two values: normal or small-caps.  For
# TrueType fonts, which are scalable fonts, small-caps is equivalent
# to using a font size of 'smaller', or about 83% of the current font
# size.
#
# The font.weight property has effectively 13 values: normal, bold,
# bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
# 400, and bold is 700.  bolder and lighter are relative values with
# respect to the current weight.
#
# The font.stretch property has 11 values: ultra-condensed,
# extra-condensed, condensed, semi-condensed, normal, semi-expanded,
# expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
# property is not currently implemented.
#
# The font.size property is the default font size for text, given in pts.
# 12pt is the standard value.
#
 font.family         : serif
#font.style          : normal
#font.variant        : normal
font.weight         : normal
#font.stretch        : normal
# note that font.size controls default text sizes.  To configure
# special text sizes tick labels, axes, labels, title, etc, see the rc
# settings for axes and ticks. Special text sizes can be defined
# relative to font.size, using the following values: xx-small, x-small,
# small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 12.0
font.serif          : Computer Modern #Times #Bitstream Vera Serif, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
#font.sans-serif     : Bitstream Vera Sans, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, Impact, Western, Humor Sans, fantasy
#font.monospace      : Bitstream Vera Sans Mono, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

### TEXT
# text properties used by text.Text.  See
# http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
# information on text properties

#text.color          : black

### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : True  # use latex for all text handling. The following fonts
                              # are supported through the usual rc parameter settings:
                              # new century schoolbook, bookman, times, palatino,
                              # zapf chancery, charter, serif, sans-serif, helvetica,
                              # avant garde, courier, monospace, computer modern roman,
                              # computer modern sans serif, computer modern typewriter
                              # If another font is desired which can loaded using the
                              # LaTeX \usepackage command, please inquire at the
                              # matplotlib mailing list
#text.latex.unicode : False # use "ucs" and "inputenc" LaTeX packages for handling
                            # unicode strings.
#text.latex.preamble : \usepackage{amsmath}
## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            # AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            # IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            # preamble is a comma separated list of LaTeX statements
                            # that are included in the LaTeX document preamble.
                            # An example:
                            # text.latex.preamble : \usepackage{bm},\usepackage{euler}
                            # The following packages are always loaded with usetex, so
                            # beware of package collisions: color, geometry, graphicx,
                            # type1cm, textcomp. Adobe Postscript (PSSNFS) font packages
                            # may also be loaded, depending on your font settings

#text.dvipnghack : None      # some versions of dvipng don't handle alpha
                             # channel properly.  Use True to correct
                             # and flush ~/.matplotlib/tex.cache
                             # before testing and False to force
                             # correction off.  None will try and
                             # guess based on your dvipng version

#text.hinting : auto   # May be one of the following:
                       #   'none': Perform no hinting
                       #   'auto': Use freetype's autohinter
                       #   'native': Use the hinting information in the
                       #             font file, if available, and if your
                       #             freetype library supports it
                       #   'either': Use the native hinting information,
                       #             or the autohinter if none is available.
                       # For backward compatibility, this value may also be
                       # True === 'auto' or False === 'none'.
#text.hinting_factor : 8 # Specifies the amount of softness for hinting in the
                         # horizontal direction.  A value of 1 will hint to full
                         # pixels.  A value of 2 will hint to half pixels etc.

#text.antialiased : True # If True (default), the text will be antialiased.
                         # This only affects the Agg backend.

# The following settings allow you to select the fonts in math mode.
# They map from a TeX font name to a fontconfig font pattern.
# These settings are only used if mathtext.fontset is 'custom'.
# Note that this "custom" mode is unsupported and may go away in the
# future.
#mathtext.cal : cursive
#mathtext.rm  : serif
#mathtext.tt  : monospace
#mathtext.it  : serif:italic
#mathtext.bf  : serif:bold
#mathtext.sf  : sans
#mathtext.fontset : cm # Should be 'cm' (Computer Modern), 'stix',
                       # 'stixsans' or 'custom'
#mathtext.fallback_to_cm : True  # When True, use symbols from the Computer Modern
                                 # fonts when a symbol can not be found in one of
                                 # the custom math fonts.

#mathtext.default : it # The default font to use for math.
                       # Can be any of the LaTeX font names, including
                       # the special name "regular" for the same font
                       # used in regular text.

### AXES
# default face and edge color, default tick sizes,
# default fontsizes for ticklabels, and so on.  See
# http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
#axes.hold           : True    # whether to clear the axes by default on
#axes.facecolor      : white   # axes background color
#axes.edgecolor      : black   # axes edge color
axes.linewidth      : 0.75     # edge linewidth
#axes.grid           : False   # display grid or not
#axes.titlesize      : large   # fontsize of the axes title
axes.labelsize      : 9  # fontsize of the x any y labels
#axes.labelpad       : 2     # space between label and axis
#axes.labelweight    : normal  # weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : False   # whether axis gridlines and ticks are below
                               # the axes elements (lines, text, etc)

#axes.formatter.limits : -7, 7 # use scientific notation if log10
                               # of the axis range is smaller than the
                               # first or larger than the second
#axes.formatter.use_locale : False # When True, format tick labels
                                   # according to the user's locale.
                                   # For example, use ',' as a decimal
                                   # separator in the fr_FR locale.
#axes.formatter.use_mathtext : False # When True, use mathtext for scientific
                                     # notation.
#axes.formatter.useoffset      : True    # If True, the tick label formatter
                                         # will default to labeling ticks relative
                                         # to an offset when the data range is very
                                         # small compared to the minimum absolute
                                         # value of the data.

#axes.unicode_minus  : True    # use unicode for the minus symbol
                               # rather than hyphen.  See
                               # http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', 'bgrcmyk')
                                            # color cycle for plot lines
                                            # as list of string colorspecs:
                                            # single letter, long name, or
                                            # web-style hex
#axes.xmargin        : 0  # x margin.  See `axes.Axes.margins`
#axes.ymargin        : 0  # y margin See `axes.Axes.margins`

#polaraxes.grid      : True    # display grid on polar axes
#axes3d.grid         : True    # display grid on 3d axes

### TICKS
# see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.major.size     : 4      # major tick size in points
xtick.minor.size     : 2      # minor tick size in points
xtick.major.width    : 0.75    # major tick width in points
xtick.minor.width    : 0.75    # minor tick width in points
xtick.major.pad      : 4      # distance to major tick label in points
#xtick.minor.pad      : 4      # distance to the minor tick label in points
#xtick.color          : k      # color of the tick labels
xtick.labelsize      : 9 # fontsize of the tick labels
xtick.direction      : in     # direction: in, out, or inout

ytick.major.size     : 5      # major tick size in points
ytick.minor.size     : 2      # minor tick size in points
ytick.major.width    : 0.75    # major tick width in points
ytick.minor.width    : 0.75    # minor tick width in points
ytick.major.pad      : 4      # distance to major tick label in points
#ytick.minor.pad      : 4      # distance to the minor tick label in points
#ytick.color          : k      # color of the tick labels
ytick.labelsize      : 9 # fontsize of the tick labels
ytick.direction      : in     # direction: in, out, or inout


### GRIDS
#grid.color       :   black   # grid color
#grid.linestyle   :   :       # dotted
#grid.linewidth   :   0.5     # in points
#grid.alpha       :   1.0     # transparency, between 0.0 and 1.0

### Legend
legend.fancybox      : True  # if True, use a rounded box for the
                               # legend, else a rectangle
#legend.isaxes        : True
#legend.numpoints     : 2      # the number of points in the legend line
legend.fontsize      : 9
#legend.borderpad     : 0.5    # border whitespace in fontsize units
#legend.markerscale   : 1.0    # the relative size of legend markers vs. original
# the following dimensions are in axes coords
legend.labelspacing  : 0.65    # the vertical space between the legend entries in fraction of fontsize
legend.handlelength  : 1.2     # the length of the legend lines in fraction of fontsize
#legend.handleheight  : 0.7     # the height of the legend handle in fraction of fontsize
#legend.handletextpad : 0.8    # the space between the legend line and legend text in fraction of fontsize
#legend.borderaxespad : 0.5   # the border between the axes and legend edge in fraction of fontsize
#legend.columnspacing : 2.    # the border between the axes and legend edge in fraction of fontsize
#legend.shadow        : False
legend.frameon       : True   # whether or not to draw a frame around legend
legend.framealpha    : None    # opacity of of legend frame
#legend.scatterpoints : 3 # number of scatter points

### FIGURE
# See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
#figure.titlesize : large # size of the figure title
#figure.titleweight : normal   # weight of the figure title
figure.figsize   : 3.3, 2.5    # figure size in inches
#figure.dpi       : 80      # figure dots per inch
#figure.facecolor : 0.75    # figure facecolor; 0.75 is scalar gray
#figure.edgecolor : white   # figure edgecolor
#figure.autolayout : False  # When True, automatically adjust subplot
                            # parameters to make the plot fit the figure
#figure.max_open_warning : 20  # The maximum number of figures to open through
                               # the pyplot interface before emitting a warning.
                               # If less than one this feature is disabled.

# The figure subplot parameters.  All dimensions are a fraction of the
# figure width or height
figure.subplot.left    : 0.11 # the left side of the subplots of the figure
figure.subplot.right   : 0.97    # the right side of the subplots of the figure
figure.subplot.bottom  : 0.08    # the bottom of the subplots of the figure
figure.subplot.top     : 0.99    # the top of the subplots of the figure
figure.subplot.wspace  : 0.50    # the amount of width reserved for blank space between subplots
figure.subplot.hspace  : 0.3   # the amount of height reserved for white space between subplots


### IMAGES
#image.aspect : equal             # equal | auto | a number
#image.interpolation  : bilinear  # see help(imshow) for options
#image.cmap   : jet               # gray | jet etc...
#image.lut    : 256               # the size of the colormap lookup table
#image.origin : upper             # lower | upper
#image.resample  : False
#image.composite_image : True     # When True, all the images on a set of axes are 
                                  # combined into a single composite image before 
                                  # saving a figure as a vector graphics file, 
                                  # such as a PDF.

### CONTOUR PLOTS
#contour.negative_linestyle : dashed # dashed | solid
#contour.corner_mask        : True   # True | False | legacy

### ERRORBAR PLOTS
#errorbar.capsize : 3             # length of end cap on error bars in pixels

### Agg rendering
### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           # 0 to disable; values in the range
                                  # 10000 to 100000 can improve speed slightly
                                  # and prevent an Agg rendering failure
                                  # when plotting very large data sets,
                                  # especially if they are very gappy.
                                  # It may cause minor artifacts, though.
                                  # A value of 20000 is probably a good
                                  # starting point.
### SAVING FIGURES
#path.simplify : True   # When True, simplify paths by removing "invisible"
                        # points to reduce file size and increase rendering
                        # speed
#path.simplify_threshold : 0.1  # The threshold of similarity below which
                                # vertices will be removed in the simplification
                                # process
#path.snap : True # When True, rectilinear axis-aligned paths will be snapped to
                  # the nearest pixel when certain criteria are met.  When False,
                  # paths will never be snapped.
#path.sketch : None # May be none, or a 3-tuple of the form (scale, length,
                    # randomness).
                    # *scale* is the amplitude of the wiggle
                    # perpendicular to the line (in pixels).  *length*
                    # is the length of the wiggle along the line (in
                    # pixels).  *randomness* is the factor by which
                    # the length is randomly scaled.

# the default savefig params can be different from the display params
# e.g., you may want a higher resolution, or to make the figure
# background white
#savefig.dpi         : 100      # figure dots per inch
#savefig.facecolor   : white    # figure facecolor when saving
#savefig.edgecolor   : white    # figure edgecolor when saving
#savefig.format      : png      # png, ps, pdf, svg
#savefig.bbox        : standard # 'tight' or 'standard'.
                                # 'tight' is incompatible with pipe-based animation
                                # backends but will workd with temporary file based ones:
                                # e.g. setting animation.writer to ffmpeg will not work,
                                # use ffmpeg_file instead
#savefig.pad_inches  : 0.1      # Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       # when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        # default directory in savefig dialog box,
                                # leave empty to always use current working directory
#savefig.transparent : False    # setting that controls whether figures are saved with a
                                # transparent background by default

# tk backend params
#tk.window_focus   : False    # Maintain shell focus for TkAgg

# ps backend params
#ps.papersize      : letter   # auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    # use of afm fonts, results in small files
#ps.usedistiller   : False    # can be: None, ghostscript or xpdf
                                          # Experimental: may produce smaller files.
                                          # xpdf intended for production of publication quality files,
                                          # but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      # dpi
#ps.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# pdf backend params
#pdf.compression   : 6 # integer from 0 to 9
                       # 0 disables compression (good for debugging)
#pdf.fonttype       : 3         # Output Type 3 (Type3) or Type 42 (TrueType)

# svg backend params
#svg.image_inline : True       # write raster image data directly into the svg file
#svg.image_noscale : False     # suppress scaling of raster data embedded in SVG
#svg.fonttype : 'path'         # How to handle SVG fonts:
#    'none': Assume fonts are installed on the machine where the SVG will be viewed.
#    'path': Embed characters as paths -- supported by most SVG renderers
#    'svgfont': Embed characters as SVG fonts -- supported only by Chrome,
#               Opera and Safari

# docstring params
#docstring.hardcopy = False  # set this when you want to generate hardcopy docstring

# Set the verbose flags.  This controls how much information
# matplotlib gives you at runtime and where it goes.  The verbosity
# levels are: silent, helpful, debug, debug-annoying.  Any level is
# inclusive of all the levels below it.  If your setting is "debug",
# you'll get all the debug and helpful messages.  When submitting
# problems to the mailing-list, please set verbose to "helpful" or "debug"
# and paste the output into your report.
#
# The "fileo" gives the destination for any calls to verbose.report.
# These objects can a filename, or a filehandle like sys.stdout.
#
# You can override the rc default verbosity from the command line by
# giving the flags --verbose-LEVEL where LEVEL is one of the legal
# levels, e.g., --verbose-helpful.
#
# You can access the verbose instance in your code
#   from matplotlib import verbose.
#verbose.level  : silent      # one of silent, helpful, debug, debug-annoying
#verbose.fileo  : sys.stdout  # a log filename, sys.stdout or sys.stderr

# Event keys to interact with figures/plots via keyboard.
# Customize these settings according to your needs.
# Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')

#keymap.fullscreen : f               # toggling
#keymap.home : h, r, home            # home or reset mnemonic
#keymap.back : left, c, backspace    # forward / backward keys to enable
#keymap.forward : right, v           #   left handed quick navigation
#keymap.pan : p                      # pan mnemonic
#keymap.zoom : o                     # zoom mnemonic
#keymap.save : s                     # saving current figure
#keymap.quit : ctrl+w, cmd+w         # close the current figure
#keymap.grid : g                     # switching on/off a grid in current axes
#keymap.yscale : l                   # toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : L, k                # toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 # enable all axes

# Control location of examples data files
#examples.directory : ''   # directory to look in for custom installation

###ANIMATION settings
#animation.html : 'none'           # How to display the animation as HTML in
                                   # the IPython notebook. 'html5' uses
                                   # HTML5 video tag.
#animation.writer : ffmpeg         # MovieWriter 'backend' to use
#animation.codec : mpeg4           # Codec to use for writing movie
#animation.bitrate: -1             # Controls size/quality tradeoff for movie.
                                   # -1 implies let utility auto-determine
#animation.frame_format: 'png'     # Controls frame format used by temp files
#animation.ffmpeg_path: 'ffmpeg'   # Path to ffmpeg binary. Without full path
                                   # $PATH is searched
#animation.ffmpeg_args: ''         # Additional arguments to pass to ffmpeg
#animation.avconv_path: 'avconv'   # Path to avconv binary. Without full path
                                   # $PATH is searched
#animation.avconv_args: ''         # Additional arguments to pass to avconv
#animation.mencoder_path: 'mencoder'
                                   # Path to mencoder binary. Without full path
                                   # $PATH is searched
#animation.mencoder_args: ''       # Additional arguments to pass to mencoder
#animation.convert_path: 'convert' # Path to ImageMagick's convert binary.
                                   # On Windows use the full path since convert
                                   # is also the name of a system tool.

